EditGAN: High-Precision Semantic Image Editing

Generative adversarial networks (GANs) have recently found applications in image editing. However, most GAN based image editing methods often require large scale datasets with semantic segmentation annotations for training, only provide high level control, or merely interpolate between different images. Here, we propose EditGAN, a novel method for high quality, high precision semantic image editing, allowing users to edit images by modifying their highly detailed part segmentation masks, e.g., drawing a new mask for the headlight of a car. EditGAN builds on a GAN framework that jointly models images and their semantic segmentations, requiring only a handful of labeled examples, making it a scalable tool for editing. Specifically, we embed an image into the GAN latent space and perform conditional latent code optimization according to the segmentation edit, which effectively also modifies the image. To amortize optimization, we find editing vectors in latent space that realize the edits. The framework allows us to learn an arbitrary number of editing vectors, which can then be directly applied on other images at interactive rates. We experimentally show that EditGAN can manipulate images with an unprecedented level of detail and freedom, while preserving full image quality.We can also easily combine multiple edits and perform plausible edits beyond EditGAN training data. We demonstrate EditGAN on a wide variety of image types and quantitatively outperform several previous editing methods on standard editing benchmark tasks.

==> doc/3_background.tex <==
%!TEX root = ../main.tex
\vspace{-2mm}{}
\section{Background}
\vspace{-1mm}

We first briefly introduce StyleGAN~\cite{karras2019style, karras2020analyzing}. The StyleGAN generator maps a latent code $z \in Z$ drawn from a normal distribution to a realistic image. Latent code $z$  is first mapped to an intermediate latent code $w \in W$ by a mapping function. $w$ is then transformed to $k$ vectors, $w^1,..., w^k$, through $k$ learned affine transformations.  These $k$ transformed latent codes are fed in synthesis blocks in a progressive fashion~\cite{karras2017progressive}.  We denote synthesis blocks as $\{Style_0, Style_1.., Style_k\}$ and the output from synthesis blocks as feature maps $\{S^0, S^1.., S^k\}$.


Recently, DatasetGAN~\cite{zhang2021datasetgan} and SemanticGAN~\cite{li2021semantic} utilized the insight of generative
models such as StyleGAN that are trained to synthesize highly realistic images must acquire semantic knowledge in their high dimensional latent space. Joint distribution of images and labels $p(x, y)$ is learned with StyleGAN. In particular, in DatasetGAN~\cite{zhang2021datasetgan}, authors built a simple three-layer MLP classifier on top of  concatenation of feature tensor $S^* = (S^{0,*}, S^{1,*}.., S^{k,*})$ to generate segmentation map $y$ together with image $x$. The author shows that such joint distribution is extremely data efficient to train, as low as 16 annotated images are needed, and generalize well across GAN's latent space.

DatasetGAN~\cite{zhang2021datasetgan} turns such joint distribution $p(x, y)$ to an infinite annotated dataset generator. In this paper, we utilize joint distribution $p(x, y)$ on the task semantic real image editing. 


% $g_\theta(\vy,  \hat\vy) \rightarrow \vy'$
